Squaring operations in the $RO(C_2)$-graded and real motivic Adams spectral sequences

In this paper we establish a formula for computing $d_2(sq^i(x))$ where $x$ is a permanent cycle in the $C_2$-equivariant Adams spectral sequence or the motivic Adams spectral sequence over $Spec(\mathbb{R})$. This requires establishing that the Adams towers have an $H_{\infty}$-structure as well as determining the attaching maps for $C_2$-equivariant projective spaces. The attaching maps of $C_2$-equivariant projective spaces can then be used to determine the coefficients of differentials in both the equivariant and motivic case. At the end some sample computations are given.

==> Bibliography.tex <==
\begin{thebibliography}{99}

@article {Caruso5,
    AUTHOR = {Caruso, Jeffrey L.},
     TITLE = {Operations in equivariant {${\bf Z}/p$}-cohomology},
   JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
  FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical
              Society},
    VOLUME = {126},
      YEAR = {1999},
    NUMBER = {3},
     PAGES = {521--541},
      ISSN = {0305-0041},
     CODEN = {MPCPCO},
   MRCLASS = {55S91 (55N91 55P42 55P91 55S10)},
  MRNUMBER = {1684248 (2000d:55028)},
MRREVIEWER = {Steven R. Costenoble},
       DOI = {10.1017/S0305004198003375},
       URL = {http://dx.doi.org/10.1017/S0305004198003375},
}

@article {ChristensenDwyerIsaksenObstModelCats,
    AUTHOR = {Christensen, J. Daniel and Dwyer, William G. and Isaksen,
              Daniel C.},
     TITLE = {Obstruction theory in model categories},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {181},
      YEAR = {2004},
    NUMBER = {2},
     PAGES = {396--416},
      ISSN = {0001-8708},
     CODEN = {ADMTA4},
   MRCLASS = {55S35 (18G30 18G55 55P42 55U35)},
  MRNUMBER = {2026865},
MRREVIEWER = {G{\'e}rald Gaudens},
       DOI = {10.1016/S0001-8708(03)00070-7},
       URL = {http://dx.doi.org/10.1016/S0001-8708(03)00070-7},
}

@article {BlumbergHillNorms,
    AUTHOR = {Blumberg, Andrew J. and Hill, Michael A.},
     TITLE = {Operadic multiplications in equivariant spectra, norms, and
              transfers},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {285},
      YEAR = {2015},
     PAGES = {658--708},
      ISSN = {0001-8708},
   MRCLASS = {55P91 (18D50 55P43 55P48)},
  MRNUMBER = {3406512},
MRREVIEWER = {Markus Szymik},
       DOI = {10.1016/j.aim.2015.07.013},
       URL = {http://dx.doi.org/10.1016/j.aim.2015.07.013},
}

@article {HHRKervaire,
    AUTHOR = {Hill, M. A. and Hopkins, M. J. and Ravenel, D. C.},
     TITLE = {On the nonexistence of elements of {K}ervaire invariant one},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {184},
      YEAR = {2016},
    NUMBER = {1},
     PAGES = {1--262},
      ISSN = {0003-486X},
   MRCLASS = {55P91 (55N22 55P42 55Q45 55T15 55U35 57R15)},
  MRNUMBER = {3505179},
       DOI = {10.4007/annals.2016.184.1.1},
       URL = {http://dx.doi.org/10.4007/annals.2016.184.1.1},
}

@article {KronholmFree,
	AUTHOR = {Kronholm, William C.},
	TITLE = {A freeness theorem for {$RO(\Bbb Z/2)$}-graded cohomology},
	JOURNAL = {Topology Appl.},
	FJOURNAL = {Topology and its Applications},
	VOLUME = {157},
	YEAR = {2010},
	NUMBER = {5},
	PAGES = {902--915},
	ISSN = {0166-8641},
	CODEN = {TIAPD9},
	MRCLASS = {55N91 (55R40)},
	MRNUMBER = {2593703},
	MRREVIEWER = {Steven R. Costenoble},
	DOI = {10.1016/j.topol.2009.12.006},
	URL = {http://dx.doi.org/10.1016/j.topol.2009.12.006},
}

@article {LewisMandellUCandKSS,
	AUTHOR = {Lewis, Jr., L. Gaunce and Mandell, Michael A.},
	TITLE = {Equivariant universal coefficient and {K}\"unneth spectral
	sequences},
	JOURNAL = {Proc. London Math. Soc. (3)},
	FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
	VOLUME = {92},
	YEAR = {2006},
	NUMBER = {2},
	PAGES = {505--544},
	ISSN = {0024-6115},
	CODEN = {PLMTAL},
	MRCLASS = {55N91 (55FP43 55U20 55U25)},
	MRNUMBER = {2205726},
	MRREVIEWER = {R. E. Stong},
	DOI = {10.1112/S0024611505015492},
	URL = {http://dx.doi.org/10.1112/S0024611505015492},
}


@article {HuKriz,
    AUTHOR = {Hu, Po and Kriz, Igor},
     TITLE = {Real-oriented homotopy theory and an analogue of the
              {A}dams-{N}ovikov spectral sequence},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {40},
      YEAR = {2001},
    NUMBER = {2},
     PAGES = {317--399},
      ISSN = {0040-9383},
     CODEN = {TPLGAF},
   MRCLASS = {55T15 (19L47 55N22 55N91 55P42 55P91)},
  MRNUMBER = {1808224},
MRREVIEWER = {J. P. C. Greenlees},
       DOI = {10.1016/S0040-9383(99)00065-8},
       URL = {http://dx.doi.org/10.1016/S0040-9383(99)00065-8},
}
		
@incollection {Robinson,
    AUTHOR = {Robinson, Alan},
     TITLE = {Classical obstructions and {$S$}-algebras},
 BOOKTITLE = {Structured ring spectra},
    SERIES = {London Math. Soc. Lecture Note Ser.},
    VOLUME = {315},
     PAGES = {133--149},
 PUBLISHER = {Cambridge Univ. Press, Cambridge},
      YEAR = {2004},
   MRCLASS = {55P43 (55S35)},
  MRNUMBER = {2122157},
MRREVIEWER = {Yutaka Hemmi},
       DOI = {10.1017/CBO9780511529955.008},
       URL = {http://dx.doi.org/10.1017/CBO9780511529955.008},
}

@article {AngeltveitKn,
    AUTHOR = {Angeltveit, Vigleik},
     TITLE = {Uniqueness of {M}orava {$K$}-theory},
   JOURNAL = {Compos. Math.},
  FJOURNAL = {Compositio Mathematica},
    VOLUME = {147},
      YEAR = {2011},
    NUMBER = {2},
     PAGES = {633--648},
      ISSN = {0010-437X},
   MRCLASS = {55N22 (18D50 55P43 55S35)},
  MRNUMBER = {2776615},
MRREVIEWER = {Richard John Steiner},
       DOI = {10.1112/S0010437X10005026},
       URL = {http://dx.doi.org/10.1112/S0010437X10005026},
}

@incollection {Lazarev,
    AUTHOR = {Lazarev, A.},
     TITLE = {Spaces of multiplicative maps between highly structured ring
              spectra},
 BOOKTITLE = {Categorical decomposition techniques in algebraic topology
              ({I}sle of {S}kye, 2001)},
    SERIES = {Progr. Math.},
    VOLUME = {215},
     PAGES = {237--259},
 PUBLISHER = {Birkh\"auser, Basel},
      YEAR = {2004},
   MRCLASS = {55P43},
  MRNUMBER = {2039769},
MRREVIEWER = {Birgit Richter},
}

@article {Caruso,
	AUTHOR = {Caruso, Jeffrey L.},
	TITLE = {Operations in equivariant {${\bf Z}/p$}-cohomology},
	JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
	FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical
	Society},
	VOLUME = {126},
	YEAR = {1999},
	NUMBER = {3},
	PAGES = {521--541},
	ISSN = {0305-0041},
	CODEN = {MPCPCO},
	MRCLASS = {55S91 (55N91 55P42 55P91 55S10)},
	MRNUMBER = {1684248},
	MRREVIEWER = {Steven R. Costenoble},
	DOI = {10.1017/S0305004198003375},
	URL = {http://dx.doi.org/10.1017/S0305004198003375},
}

@article {Bredon,
    AUTHOR = {Bredon, G. E.},
     TITLE = {Equivariant stable stems},
   JOURNAL = {Bull. Amer. Math. Soc.},
  FJOURNAL = {Bulletin of the American Mathematical Society},
    VOLUME = {73},
      YEAR = {1967},
     PAGES = {269--273},
      ISSN = {0002-9904},
   MRCLASS = {55.40},
  MRNUMBER = {0206947 (34 \#6763)},
MRREVIEWER = {N. Stein},
}

@article {BrunerInfiniteFamily,
	AUTHOR = {Bruner, Robert R.},
	TITLE = {An infinite family in {$\pi \sb\ast S^{0}$} derived from
	{M}ahowald's {$\eta _{j}$} family},
	JOURNAL = {Proc. Amer. Math. Soc.},
	FJOURNAL = {Proceedings of the American Mathematical Society},
	VOLUME = {82},
	YEAR = {1981},
	NUMBER = {4},
	PAGES = {637--639},
	ISSN = {0002-9939},
	CODEN = {PAMYAR},
	MRCLASS = {55Q45 (55Q35)},
	MRNUMBER = {614893},
	MRREVIEWER = {M. Mahowald},
	DOI = {10.2307/2043786},
	URL = {http://dx.doi.org/10.2307/2043786},
}

@article {BrunerNewDifferential,
	AUTHOR = {Bruner, Robert},
	TITLE = {A new differential in the {A}dams spectral sequence},
	JOURNAL = {Topology},
	FJOURNAL = {Topology. An International Journal of Mathematics},
	VOLUME = {23},
	YEAR = {1984},
	NUMBER = {3},
	PAGES = {271--276},
	ISSN = {0040-9383},
	CODEN = {TPLGAF},
	MRCLASS = {55Q45 (55T15)},
	MRNUMBER = {770563},
	MRREVIEWER = {Stanley Kochman},
	DOI = {10.1016/0040-9383(84)90010-7},
	URL = {http://dx.doi.org/10.1016/0040-9383(84)90010-7},
}

@article {BalmerSSS,
    AUTHOR = {Balmer, Paul},
     TITLE = {Spectra, spectra, spectra---tensor triangular spectra versus
              {Z}ariski spectra of endomorphism rings},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {10},
      YEAR = {2010},
    NUMBER = {3},
     PAGES = {1521--1563},
      ISSN = {1472-2747},
   MRCLASS = {18E30 (19K56 55U35)},
  MRNUMBER = {2661535},
MRREVIEWER = {Amnon Neeman},
       DOI = {10.2140/agt.2010.10.1521},
       URL = {http://dx.doi.org/10.2140/agt.2010.10.1521},
}

@article {DwilsonEquivDL,
	AUTHOR = {Wilson, Dylan},
	TITLE = {Power operations for ${\mathrm{{H}}\mathbb{F}}\sb 2$ and a cellular construction of ${\mathrm{{B}}\mathrm{{P}}}\mathbb{R}$},
	JOURNAL = {},
	FJOURNAL = {},
	VOLUME = {},
	YEAR = {2010},
	NUMBER = {},
	PAGES = {},
	ISSN = {},
	MRCLASS = {},
	MRNUMBER = {},
	MRREVIEWER = {},
	DOI = {},
	URL = {http://arxiv.org/abs/1611.06958},
}

@article {Spitzweck,
	AUTHOR = {Spitzweck, Markus},
	TITLE = {Derived {F}undamental {G}roups for {T}ate {M}otives},
	JOURNAL = {},
	FJOURNAL = {},
	VOLUME = {},
	YEAR = {2010},
	NUMBER = {},
	PAGES = {},
	ISSN = {},
	MRCLASS = {},
	MRNUMBER = {},
	MRREVIEWER = {},
	DOI = {},
	URL = {http://arxiv.org/abs/1005.2670},
}

@article {KSSpaper,
    AUTHOR = {Tilson, Sean},
     TITLE = {Power operations in the {K}\"unneth spectral sequence and commutative {H}{F}p-algebras},
   JOURNAL = {},
  FJOURNAL = {},
    VOLUME = {},
      YEAR = {2016},
    NUMBER = {},
     PAGES = {},
      ISSN = {},
   MRCLASS = {},
  MRNUMBER = {},
MRREVIEWER = {},
       DOI = {},
       URL = {http://arxiv.org/abs/1602.06736},
}

@article {DwyerF2,
	AUTHOR = {Dwyer, W. G.},
	TITLE = {Homotopy operations for simplicial commutative algebras},
	JOURNAL = {Trans. Amer. Math. Soc.},
	FJOURNAL = {Transactions of the American Mathematical Society},
	VOLUME = {260},
	YEAR = {1980},
	NUMBER = {2},
	PAGES = {421--435},
	ISSN = {0002-9947},
	CODEN = {TAMTAM},
	MRCLASS = {55S20 (18G30)},
	MRNUMBER = {574789},
	MRREVIEWER = {Howard Lyn Hiller},
	DOI = {10.2307/1998012},
	URL = {http://dx.doi.org/10.2307/1998012},
}

@article {slicemult,
	AUTHOR = {Guti{\'e}rrez, Javier J. and R{\"o}ndigs, Oliver and
	Spitzweck, Markus and {\O}stv{\ae}r, Paul Arne},
	TITLE = {Motivic slices and coloured operads},
	JOURNAL = {J. Topol.},
	FJOURNAL = {Journal of Topology},
	VOLUME = {5},
	YEAR = {2012},
	NUMBER = {3},
	PAGES = {727--755},
	ISSN = {1753-8416},
	MRCLASS = {14F42 (18D50 55P43)},
	MRNUMBER = {2971612},
	MRREVIEWER = {Daniel C. Isaksen},
	DOI = {10.1112/jtopol/jts015},
	URL = {http://dx.doi.org/10.1112/jtopol/jts015},
}

		
@article {HopkinsLawson,
    AUTHOR = {Hopkins, Michael J. and Lawson, Tyler},
     TITLE = {Strictly commtuative complex orientation theory},
   JOURNAL = {},
  FJOURNAL = {},
    VOLUME = {},
      YEAR = {2016},
    NUMBER = {},
     PAGES = {},
      ISSN = {},
   MRCLASS = {},
  MRNUMBER = {},
MRREVIEWER = {},
       DOI = {},
       URL = {http://arxiv.org/abs/1603.00047},
}

@article {LigaardMadsen,
    AUTHOR = {Ligaard, Hans and Madsen, Ib},
     TITLE = {Homology operations in the {E}ilenberg-{M}oore spectral
              sequence},
   JOURNAL = {Math. Z.},
  FJOURNAL = {Mathematische Zeitschrift},
    VOLUME = {143},
      YEAR = {1975},
     PAGES = {45--54},
      ISSN = {0025-5874},
   MRCLASS = {55H20},
  MRNUMBER = {0375316},
MRREVIEWER = {J. P. May},
}

@article {HillLawson,
    AUTHOR = {Hill, M. and Lawson, T.},
     TITLE = {Topological modular forms with level structure},
   JOURNAL = {},
  FJOURNAL = {},
    VOLUME = {},
      YEAR = {2015},
    NUMBER = {},
     PAGES = {},
      ISSN = {},
   MRCLASS = {},
  MRNUMBER = {},
MRREVIEWER = {},
       DOI = {},
       URL = {http://www.math.umn.edu/~tlawson/papers/logetaletmf.pdf},
}

@article {LawsonNaumann,
    AUTHOR = {Lawson, T. and Naumann, N.},
     TITLE = {Commutativity conditions for truncated {B}rown-{P}eterson
              spectra of height 2},
   JOURNAL = {J. Topol.},
  FJOURNAL = {Journal of Topology},
    VOLUME = {5},
      YEAR = {2012},
    NUMBER = {1},
     PAGES = {137--168},
      ISSN = {1753-8416},
   MRCLASS = {55P42 (55N22 55N34 55P43)},
  MRNUMBER = {2897051},
MRREVIEWER = {Rui Miguel Saramago},
       DOI = {10.1112/jtopol/jtr030},
       URL = {http://dx.doi.org/10.1112/jtopol/jtr030},
}

@article {BrunerRognes,
    AUTHOR = {Bruner, R. R. and Rognes, J.},
     TITLE = {Differentials in the homological homotopy fixed point spectral
              sequence},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {5},
      YEAR = {2005},
     PAGES = {653--690 (electronic)},
      ISSN = {1472-2747},
   MRCLASS = {19D55 (55P43 55P91 55S12 55T05)},
  MRNUMBER = {2153113 (2007d:19003)},
       DOI = {10.2140/agt.2005.5.653},
       URL = {http://dx.doi.org/10.2140/agt.2005.5.653},
       }
@article {BakerGilmourReinhard,
    AUTHOR = {Baker, A. and Gilmour, H. and Reinhard, P.},
     TITLE = {Topological {A}ndr\'e-{Q}uillen homology for cellular
              commutative {$S$}-algebras},
   JOURNAL = {Abh. Math. Semin. Univ. Hambg.},
  FJOURNAL = {Abhandlungen aus dem Mathematischen Seminar der Universit\"at
              Hamburg},
    VOLUME = {78},
      YEAR = {2008},
    NUMBER = {1},
     PAGES = {27--50},
      ISSN = {0025-5858},
   MRCLASS = {55P43 (13D03 55N35)},
  MRNUMBER = {2501527 (2010c:55006)},
MRREVIEWER = {Srikanth B. Iyengar},
       DOI = {10.1007/s12188-008-0005-9},
       URL = {http://dx.doi.org/10.1007/s12188-008-0005-9},
}


@article {BasterraThesis,
    AUTHOR = {Basterra, M.},
     TITLE = {Andr\'e-{Q}uillen cohomology of commutative {$S$}-algebras},
   JOURNAL = {J. Pure Appl. Algebra},
  FJOURNAL = {Journal of Pure and Applied Algebra},
    VOLUME = {144},
      YEAR = {1999},
    NUMBER = {2},
     PAGES = {111--143},
      ISSN = {0022-4049},
     CODEN = {JPAAA2},
   MRCLASS = {55P43 (13D03 18G40 55P42 55U35)},
  MRNUMBER = {1732625 (2001b:55025)},
MRREVIEWER = {Kathryn P. Hess},
       DOI = {10.1016/S0022-4049(98)00051-6},
       URL = {http://dx.doi.org/10.1016/S0022-4049(98)00051-6},
}

@book {HRS,
    AUTHOR = {Bruner, R. R. and May, J. P. and McClure, J. E. and
              Steinberger, M.},
     TITLE = {{$H\sb \infty $} ring spectra and their applications},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {1176},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin},
      YEAR = {1986},
     PAGES = {viii+388},
      ISBN = {3-540-16434-0},
   MRCLASS = {55-02 (55P42 55Sxx)},
  MRNUMBER = {836132 (88e:55001)},
MRREVIEWER = {Haynes R. Miller},
}

@book {EKMM,
    AUTHOR = {Elmendorf, A. D. and Kriz, I. and Mandell, M. A. and May, J.
              P.},
     TITLE = {Rings, modules, and algebras in stable homotopy theory},
    SERIES = {Mathematical Surveys and Monographs},
    VOLUME = {47},
      NOTE = {With an appendix by M. Cole},
 PUBLISHER = {American Mathematical Society},
   ADDRESS = {Providence, RI},
      YEAR = {1997},
     PAGES = {xii+249},
      ISBN = {0-8218-0638-6},
   MRCLASS = {55N20 (19D10 19D55 55P42 55T25)},
  MRNUMBER = {1417719 (97h:55006)},
MRREVIEWER = {Donald M. Davis},
}

@book {GreenBook,
    AUTHOR = {Ravenel, Douglas C.},
     TITLE = {Complex cobordism and stable homotopy groups of spheres},
    SERIES = {Pure and Applied Mathematics},
    VOLUME = {121},
 PUBLISHER = {Academic Press Inc.},
   ADDRESS = {Orlando, FL},
      YEAR = {1986},
     PAGES = {xx+413},
      ISBN = {0-12-583430-6; 0-12-583431-4},
   MRCLASS = {55-02 (55Qxx 57-02)},
  MRNUMBER = {860042 (87j:55003)},
MRREVIEWER = {Joseph Neisendorfer},
}

@book {Alaska,
    AUTHOR = {May, J. P.},
     TITLE = {Equivariant homotopy and cohomology theory},
    SERIES = {CBMS Regional Conference Series in Mathematics},
    VOLUME = {91},
      NOTE = {With contributions by M. Cole, G. Comeza{\~n}a, S. Costenoble,
              A. D. Elmendorf, J. P. C. Greenlees, L. G. Lewis, Jr., R. J.
              Piacenza, G. Triantafillou, and S. Waner},
 PUBLISHER = {Published for the Conference Board of the Mathematical
              Sciences, Washington, DC},
      YEAR = {1996},
     PAGES = {xiv+366},
      ISBN = {0-8218-0319-0},
   MRCLASS = {55P91 (18G99 55N91 55U35)},
  MRNUMBER = {1413302 (97k:55016)},
MRREVIEWER = {Ian Hambleton},
}

@book {LMS,
    AUTHOR = {Lewis, Jr., L. G. and May, J. P. and Steinberger, M. and
              McClure, J. E.},
     TITLE = {Equivariant stable homotopy theory},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {1213},
      NOTE = {With contributions by J. E. McClure},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin},
      YEAR = {1986},
     PAGES = {x+538},
      ISBN = {3-540-16820-6},
   MRCLASS = {55-02 (55Nxx 55Pxx 57S99)},
  MRNUMBER = {866482 (88e:55002)},
MRREVIEWER = {T. tom Dieck},
}

@article {DuggerIsaksenAdams,
    AUTHOR = {Dugger, D. and Isaksen, D.},
     TITLE = {The motivic {A}dams spectral sequence},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry \& Topology},
    VOLUME = {14},
      YEAR = {2010},
    NUMBER = {2},
     PAGES = {967--1014},
      ISSN = {1465-3060},
   MRCLASS = {55T15 (14F42 55P42)},
  MRNUMBER = {2629898 (2011e:55024)},
MRREVIEWER = {Markus Szymik},
       DOI = {10.2140/gt.2010.14.967},
       URL = {http://dx.doi.org/10.2140/gt.2010.14.967},
}

@article {DuggerIsaksenBook,
    AUTHOR = {Dugger, D. and Isaksen, D.},
     TITLE = {Fundamentals of motivic stable homotopy groups},
   JOURNAL = {},
  FJOURNAL = {},
    VOLUME = {},
      YEAR = {},
    NUMBER = {},
     PAGES = {},
      ISSN = {},
   MRCLASS = {},
  MRNUMBER = {},
MRREVIEWER = {},
       DOI = {},
       URL = {},
}
@article {StricklandMU,
    AUTHOR = {Strickland, N. P.},
     TITLE = {Products on {${\rm MU}$}-modules},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {351},
      YEAR = {1999},
    NUMBER = {7},
     PAGES = {2569--2606},
      ISSN = {0002-9947},
     CODEN = {TAMTAM},
   MRCLASS = {55N22 (55N20)},
  MRNUMBER = {1641115 (2000b:55003)},
MRREVIEWER = {W. Stephen Wilson},
       DOI = {10.1090/S0002-9947-99-02436-8},
       URL = {http://dx.doi.org/10.1090/S0002-9947-99-02436-8},
}

@article {BakerRichterAdams,
    AUTHOR = {Baker, A. and Richter, B.},
     TITLE = {On the cooperation algebra of the connective {A}dams summand},
   JOURNAL = {Tbil. Math. J.},
  FJOURNAL = {Tbilisi Mathematical Journal},
    VOLUME = {1},
      YEAR = {2008},
     PAGES = {33--70},
      ISSN = {1875-158X},
   MRCLASS = {55P43 (18G15 55N15 55N20)},
  MRNUMBER = {2434436 (2009d:55012)},
MRREVIEWER = {Donald M. Davis},
}

@article {JNobstruction,
    AUTHOR = {Johnson, N. and Noel, J.},
     TITLE = {Lifting homotopy {T}-algebra maps to strict maps},
   JOURNAL = {http://arxiv.org/abs/1301.1511},
  FJOURNAL = {}
    VOLUME = {}
      YEAR = {}
    NUMBER = {}
     PAGES = {}
      ISSN = {}
     CODEN = {}
   MRCLASS = {}
  MRNUMBER = {}
MRREVIEWER = {}
       DOI = {}
       URL = {http://arxiv.org/abs/1301.1511},
}

@article {AntieauBarthelGepner,
    AUTHOR = {Antieau, Barthel, and Gepner},
     TITLE = {On localization sequences in the algebraic K-theory of
     ring spectra},
   JOURNAL = {http://arxiv.org/abs/1412.4041},
  FJOURNAL = {}
    VOLUME = {}
      YEAR = {}
    NUMBER = {}
     PAGES = {}
      ISSN = {}
     CODEN = {}
   MRCLASS = {}
  MRNUMBER = {}
MRREVIEWER = {}
       DOI = {}
       URL = {http://arxiv.org/abs/1412.4041},
}

@article {BakerBP,
    AUTHOR = {Baker, A.},
     TITLE = {B{P}: {C}lose encounters of the ${E}_{\infty}$ kind},
   JOURNAL = {http://arxiv.org/abs/1204.4878},
  FJOURNAL = {}
    VOLUME = {}
      YEAR = {}
    NUMBER = {}
     PAGES = {}
      ISSN = {}
     CODEN = {}
   MRCLASS = {}
  MRNUMBER = {}
MRREVIEWER = {}
       DOI = {}
       URL = {http://arxiv.org/abs/1204.4878},
}

@article {BakerTAQI,
    AUTHOR = {Baker, A.},
     TITLE = {Calculating with topological {A}ndr\'e-{Q}uillen theory, {I}: {H}omotopical properties of universal derivations and free commutative ${S}$-algebras},
   JOURNAL = {http://arxiv.org/abs/1208.1868},
  FJOURNAL = {}
    VOLUME = {}
      YEAR = {}
    NUMBER = {}
     PAGES = {}
      ISSN = {}
     CODEN = {}
   MRCLASS = {}
  MRNUMBER = {}
MRREVIEWER = {}
       DOI = {}
       URL = {http://arxiv.org/abs/1208.1868},
}

@article {BousfieldKanUniversal,
    AUTHOR = {Bousfield, A. K. and Kan, D. M.},
     TITLE = {A second quadrant homotopy spectral sequence},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {177},
      YEAR = {1973},
     PAGES = {305--318},
      ISSN = {0002-9947},
   MRCLASS = {55H15},
  MRNUMBER = {0372859 (51 \#9063)},
MRREVIEWER = {Donald M. Davis},
}

@article {HackneyOpsInfLoopSpace,
    AUTHOR = {Hackney, P.},
     TITLE = {Operations in the homology spectral sequence of a cosimplicial
              infinite loop space},
   JOURNAL = {J. Pure Appl. Algebra},
  FJOURNAL = {Journal of Pure and Applied Algebra},
    VOLUME = {217},
      YEAR = {2013},
    NUMBER = {7},
     PAGES = {1350--1377},
      ISSN = {0022-4049},
     CODEN = {JPAAA2},
   MRCLASS = {55S12},
  MRNUMBER = {3019742},
       DOI = {10.1016/j.jpaa.2012.10.002},
       URL = {http://dx.doi.org/10.1016/j.jpaa.2012.10.002},
}

@article {DuggerMultSS,
    AUTHOR = {Dugger, D.},
     TITLE = {Multiplicative structures on homotopy spectral sequences I},
   JOURNAL = {http://http://pages.uoregon.edu/ddugger/mult.html},
  FJOURNAL = {},
    VOLUME = {},
      YEAR = {},
    NUMBER = {},
     PAGES = {},
      ISSN = {},
     CODEN = {},
   MRCLASS = {},
  MRNUMBER = {},
MRREVIEWER = {},
       DOI = {},
       URL = {http://http://pages.uoregon.edu/ddugger/mult.html},
}

@article {MayTraces,
    AUTHOR = {May, J. P.},
     TITLE = {The additivity of traces in triangulated categories},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {163},
      YEAR = {2001},
    NUMBER = {1},
     PAGES = {34--73},
      ISSN = {0001-8708},
     CODEN = {ADMTA4},
   MRCLASS = {18E30 (18D10)},
  MRNUMBER = {1867203 (2002k:18019)},
MRREVIEWER = {Paul Balmer},
       DOI = {10.1006/aima.2001.1995},
       URL = {http://dx.doi.org/10.1006/aima.2001.1995},
}

@book {TilsonThesis,
    AUTHOR = {Tilson, S.},
     TITLE = {P{OWER} {OPERATIONS} {IN} {THE} {K\"UNNETH} {AND}             {$C_2$-EQUIVARIANT} {ADAMS} {SPECTRAL} {SEQUENCES}},
      NOTE = {Thesis (Ph.D.)--Wayne State University},
 PUBLISHER = {ProQuest LLC, Ann Arbor, MI},
      YEAR = {2013},
     PAGES = {(no paging)},
   MRCLASS = {Thesis},
  MRNUMBER = {?},
       URL =
              {??},
}

@book {BrunerThesis,
    AUTHOR = {Bruner, R. R.},
     TITLE = {T{HE} {ADAMS} {SPECTRAL} {SEQUENCE} {OF} {$H_{\infty}$}
              {RING} {SPECTRA}},
      NOTE = {Thesis (Ph.D.)--The University of Chicago},
 PUBLISHER = {ProQuest LLC, Ann Arbor, MI},
      YEAR = {1977},
     PAGES = {(no paging)},
   MRCLASS = {Thesis},
  MRNUMBER = {2611760},
       URL =
              {http://gateway.proquest.com/openurl?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:dissertation&res_dat=xri:pqdiss&rft_dat=xri:pqdiss:T-26567},
}

@article {MilnorSteenrod,
    AUTHOR = {Milnor, J.},
     TITLE = {The {S}teenrod algebra and its dual},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {67},
      YEAR = {1958},
     PAGES = {150--171},
      ISSN = {0003-486X},
   MRCLASS = {55.00 (18.00)},
  MRNUMBER = {0099653 (20 \#6092)},
MRREVIEWER = {G. Hirsch},
}

@incollection {MaySteenrod,
    AUTHOR = {May, J. P.},
     TITLE = {A general algebraic approach to {S}teenrod operations},
 BOOKTITLE = {The {S}teenrod {A}lgebra and its {A}pplications ({P}roc.
              {C}onf. to {C}elebrate {N}. {E}. {S}teenrod's {S}ixtieth
              {B}irthday, {B}attelle {M}emorial {I}nst., {C}olumbus, {O}hio,
              1970)},
    SERIES = {Lecture Notes in Mathematics, Vol. 168},
     PAGES = {153--231},
 PUBLISHER = {Springer},
   ADDRESS = {Berlin},
      YEAR = {1970},
   MRCLASS = {55.34 (18.00)},
  MRNUMBER = {0281196 (43 \#6915)},
MRREVIEWER = {W. D. Barcus},
}

@book {Weibel,
    AUTHOR = {Weibel, C.},
     TITLE = {An introduction to homological algebra},
    SERIES = {Cambridge Studies in Advanced Mathematics},
    VOLUME = {38},
 PUBLISHER = {Cambridge University Press},
   ADDRESS = {Cambridge},
      YEAR = {1994},
     PAGES = {xiv+450},
      ISBN = {0-521-43500-5; 0-521-55987-1},
   MRCLASS = {18-01 (16-01 17-01 20-01 55Uxx)},
  MRNUMBER = {1269324 (95f:18001)},
MRREVIEWER = {Kenneth A. Brown},
}

@article {Tate,
    AUTHOR = {Tate, J.},
     TITLE = {Homology of {N}oetherian rings and local rings},
   JOURNAL = {Illinois J. Math.},
  FJOURNAL = {Illinois Journal of Mathematics},
    VOLUME = {1},
      YEAR = {1957},
     PAGES = {14--27},
      ISSN = {0019-2082},
   MRCLASS = {18.0X},
  MRNUMBER = {0086072 (19,119b)},
MRREVIEWER = {D. Buchsbaum},
}

@article {BakerLazarev,
    AUTHOR = {Baker, A. and Lazarev, A.},
     TITLE = {On the {A}dams spectral sequence for {$R$}-modules},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {1},
      YEAR = {2001},
     PAGES = {173--199},
      ISSN = {1472-2747},
   MRCLASS = {55P42 (55N20 55P43 55T15)},
  MRNUMBER = {1823498 (2002a:55011)},
MRREVIEWER = {Mark Hovey},
       DOI = {10.2140/agt.2001.1.173},
       URL = {http://dx.doi.org/10.2140/agt.2001.1.173},
}

@article {MandellTAQ,
    AUTHOR = {Mandell, M. A.},
     TITLE = {Topological {A}ndr\'e-{Q}uillen cohomology and {$E_\infty$}
              {A}ndr\'e-{Q}uillen cohomology},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {177},
      YEAR = {2003},
    NUMBER = {2},
     PAGES = {227--279},
      ISSN = {0001-8708},
     CODEN = {ADMTA4},
   MRCLASS = {55P43 (18D50 18G55)},
  MRNUMBER = {1990939 (2004d:55010)},
MRREVIEWER = {Paul G. Goerss},
       DOI = {10.1016/S0001-8708(02)00017-8},
       URL = {http://dx.doi.org/10.1016/S0001-8708(02)00017-8},
}

@incollection {BoardmanCCSS,
    AUTHOR = {Boardman, J. M.},
     TITLE = {Conditionally convergent spectral sequences},
 BOOKTITLE = {Homotopy invariant algebraic structures ({B}altimore, {MD},
              1998)},
    SERIES = {Contemp. Math.},
    VOLUME = {239},
     PAGES = {49--84},
 PUBLISHER = {Amer. Math. Soc.},
   ADDRESS = {Providence, RI},
      YEAR = {1999},
   MRCLASS = {55T05 (18A30 18G40)},
  MRNUMBER = {1718076 (2000m:55024)},
MRREVIEWER = {John McCleary},
       DOI = {10.1090/conm/239/03597},
       URL = {http://dx.doi.org/10.1090/conm/239/03597},
}

@BOOK{AdLie,
author  = {J.F. Adams},
title = {Lectures on Lie groups},
publisher = {W.A. Benjamin
(Reprinted by the University of Chicago Press, 1982)},
year={1969}
}

@BOOK{SpringerVol36,
author  = {Armand Borel},
title = {xxx},
publisher = {Springer-Verlag},
series={Lecture Notes in Mathematics},
volume = {36},
year={19XX}
}

@BOOK{BrTD,
author = {T. Br\"ocker and T. tom Dieck},
title = {Representations of compact Lie groups},
publisher = {Springer-Verlag},
year = {1985},
}

@unpublished{CM,
author = {H. Cartan and J.C. Moore},
title = {P\'eriodicit\'e des groupes d'homotopie stables des
groupes classiques, d'apr\`es Bott},
note = {S\'eminaire Henri
Cartan 1959/60. \'Ecole Normale Sup\'erieure.},
year = {1961},
}


@book{Chev,
author = {C. Chevalley},
title = {Theory of Lie groups},
publisher = {Princeton University Press},
year={1946}
}

@Book{FP,
author = {R. Fritsch and R.A. Piccinini},
title = {Cellular structures in topology},
publisher = {Cambridge University Press},
year = {1990}
}

@book{Hu,
author = {D. Husemoller},
title = {Fiber bundles},
publisher = {Springer-Verlag 
(Second edition, 1975)},
year = {1966},
}


@book{Knapp:1986,
author = {Anthony Knapp},
title = {Representation theory of semisimple groups},
publisher = {Princeton University Press},
year = {1986}
}


@book{Concise,
author = {J.P. May},
title = {A concise course in algebraic topology},
publisher = {University of Chicago Press},
year = {1999}
}

@article{MiCW,
author = {J. Milnor},
title = {On spaces having the homotopy type of a CW-complex},
journal = {Trans. Amer. Math. Soc.},
volume = {90},
year = {1959},
pages = {272--280}
}

@article{Schon,
author = {R. Schon},
title = {Fibrations over a CWh-space},
journal = {Proc. Amer. Math. Soc},
volume = {62},
year = {1976}, 
pages = {165--166},
}

@book{St,
author = {N.E. Steenrod},
title = {The topology of fiber bundles},
publisher = {Princeton University Press},
year = {1951}
}

@article{May:75,
    AUTHOR = {May, J. Peter},
     TITLE = {Classifying spaces and fibrations},
   JOURNAL = {Mem. Amer. Math. Soc.},
    VOLUME = {1},
      YEAR = {1975},
    NUMBER = {1, 155},
     PAGES = {xiii+98},
}

@article{Dol:63,
    AUTHOR = {Dold, Albrecht},
     TITLE = {Partitions of unity in the theory of fibrations},
   JOURNAL = {Ann. of Math. (2)},
    VOLUME = {78},
      YEAR = {1963},
     PAGES = {223--255},
}

@article{tom:66,
    AUTHOR = {tom Dieck, Tammo},
     TITLE = {Klassifikation numerierbarer {B}\"undel},
   JOURNAL = {Arch. Math. (Basel)},
    VOLUME = {17},
      YEAR = {1966},
     PAGES = {395--399},
}

@book{Whi:78,
    AUTHOR = {Whitehead, George W.},
     TITLE = {Elements of homotopy theory},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {61},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {New York},
      YEAR = {1978},
}

@article{Miy:52,
	author = {Miyazaki, Hiroshi},
	title = {The paracompactness of CW-complexes},
	journal = {Tohoku Math. J.},
	volume = {4},
	year = {1952},
	pages = {309--313},
}


